Closed-Loop Identification of Stabilized Models Using Dual Input-Output Parameterization

This paper introduces a dual input-output parameterization (dual IOP) for the identification of linear time-invariant systems from closed-loop data. It draws inspiration from the recent input-output parameterization developed to synthesize a stabilizing controller. The controller is parameterized in terms of closed-loop transfer functions, from the external disturbances to the input and output of the system, constrained to lie in a given subspace. Analogously, the dual IOP method parameterizes the unknown plant with analogous closed-loop transfer functions, also referred to as dual parameters. In this case, these closed-loop transfer functions are constrained to lie in an affine subspace guaranteeing that the identified plant is \emph{stabilized} by the known controller. Compared with existing closed-loop identification techniques guaranteeing closed-loop stability, such as the dual Youla parameterization, the dual IOP neither requires a doubly-coprime factorization of the controller nor a nominal plant that is stabilized by the controller. The dual IOP does not depend on the order and the state-space realization of the controller either, as in the dual system-level parameterization. Simulation shows that the dual IOP outperforms the existing benchmark methods.

==> sections/09_app.tex <==
\section*{Appendix}
\subsection{Proof of the Affine Constraints}
Starting with the following definitions,
\begin{equation}
    \begin{aligned}
        \mathbf{W} & = (I-\mathbf{GK})^{-1} \\
        \mathbf{X} & = (I-\mathbf{GK})^{-1}\mathbf{G} = \mathbf{G}(I-\mathbf{KG})^{-1} \\
        \mathbf{Y} & = (I-\mathbf{KG})^{-1}\mathbf{K} = \mathbf{K}(I-\mathbf{GK})^{-1} \\
        \mathbf{Z} & = (I-\mathbf{KG})^{-1} \\
    \end{aligned}
\end{equation}

We have, 
\begin{equation}
    \begin{aligned}
        \mathbf{Y}-\mathbf{KW} 
        & = \mathbf{K}(I-\mathbf{GK})^{-1} - \mathbf{K}(I-\mathbf{GK})^{-1} \\ 
        & = 0\\
       \mathbf{Z}-\mathbf{KX} 
        & = (I-\mathbf{KG})^{-1} - \mathbf{KG}(I-\mathbf{KG})^{-1}\\ 
        & =  (I-\mathbf{KG})(I-\mathbf{KG})^{-1} \\
        & = I\\
       \mathbf{W}-\mathbf{XK} 
        & = (I-\mathbf{GK})^{-1} - (I-\mathbf{GK})^{-1}\mathbf{GK} \\ 
        & =  (I-\mathbf{GK})^{-1}(I-\mathbf{GK}) \\
        & = I\\
       \mathbf{Y}-\mathbf{ZK} 
        & = (I-\mathbf{KG})^{-1}\mathbf{K} -(I-\mathbf{KG})^{-1}\mathbf{K} \\
        & = 0 
\end{aligned}
\end{equation}
We conclude the affine constraints in Eq.\ref{eq:4affine} are true for any arbitrary systems. 

\subsection{Proof of Theorem \ref{thm:thm2}}
The statement 1) of Theorem \ref{thm:thm2} is obviously true since the expressions of such $(\mathbf{W},\mathbf{X},\mathbf{Y},\mathbf{Z})$ are already provided in Eq.\ref{eq:XWYZ} with the affine relationship proved in Appendix A. To further prove statement 2), suppose $(\hat{\mathbf{W}}$, $\hat{\mathbf{X}}$, $\hat{\mathbf{Y}}$, $\hat{\mathbf{Z}})$ are some identified transfer functions satisfying the affine constraints, and let $\hat{\mathbf{G}} = \hat{\mathbf{W}}^{-1}\hat{\mathbf{X}}$ as the estimated plant. Then, the estimated closed-loop transfer function $\hat{\mathbf{T}}_{yr}$ from $\mathbf{r}$ to $\mathbf{y}$ is given by,
\begin{equation}
\begin{aligned}
       \hat{\mathbf{T}}_{yr} 
       & = (I-\hat{\mathbf{G}}\mathbf{K})^{-1}\hat{\mathbf{G}} \\
       & = (I-\hat{\mathbf{W}}^{-1}\hat{\mathbf{X}}\mathbf{K})^{-1}\hat{\mathbf{W}}^{-1}\hat{\mathbf{X}} \\
       & = (\hat{\mathbf{W}} - \hat{\mathbf{X}}\mathbf{K})^{-1}\hat{\mathbf{W}}\cdot \hat{\mathbf{W}}^{-1}\hat{\mathbf{X}} \\ 
       & = \hat{\mathbf{X}} \in \mathcal{RH}_\infty
\end{aligned}
\end{equation}
Thus, the transfer function from $\mathbf{r}$ to $\mathbf{y}$ is guaranteed to be stable, and similar to the other three transfer functions. The proof regarding the alternative expression $\hat{\mathbf{G}}=\hat{\mathbf{X}}\hat{\mathbf{Z}}^{-1}$ is also identical thus omitted here.


